Exploration with Limited Memory: Streaming Algorithms for Coin Tossing, Noisy Comparisons, and Multi-Armed Bandits

Consider the following abstract coin tossing problem: Given a set of $n$ coins with unknown biases, find the most biased coin using a minimal number of coin tosses. This is a common abstraction of various exploration problems in theoretical computer science and machine learning and has been studied extensively over the years. In particular, algorithms with optimal sample complexity (number of coin tosses) have been known for this problem for quite some time. Motivated by applications to processing massive datasets, we study the space complexity of solving this problem with optimal number of coin tosses in the streaming model. In this model, the coins are arriving one by one and the algorithm is only allowed to store a limited number of coins at any point -- any coin not present in the memory is lost and can no longer be tossed or compared to arriving coins. Prior algorithms for the coin tossing problem with optimal sample complexity are based on iterative elimination of coins which inherently require storing all the coins, leading to memory-inefficient streaming algorithms. We remedy this state-of-affairs by presenting a series of improved streaming algorithms for this problem: we start with a simple algorithm which require storing only $O(\log{n})$ coins and then iteratively refine it further and further, leading to algorithms with $O(\log\log{(n)})$ memory, $O(\log^*{(n)})$ memory, and finally a one that only stores a single extra coin in memory -- the same exact space needed to just store the best coin throughout the stream. Furthermore, we extend our algorithms to the problem of finding the $k$ most biased coins as well as other exploration problems such as finding top-$k$ elements using noisy comparisons or finding an $\epsilon$-best arm in stochastic multi-armed bandits, and obtain efficient streaming algorithms for these problems.

==> app-main-alg.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex


\section{Missing Details from \Cref{sec:main}}\label{app:main}

\subsection*{Proof of \Cref{clm:main-sample}}
\begin{claim*}
	The total number of coin tosses by the algorithm is at most $4n \cdot b = O(\frac{n}{\Delta^2} \cdot \log{(1/\delta)})$. 
\end{claim*}
\begin{proof}
	Each arriving coin in the stream increases the budget by $b$ and each time we make a new $\king$ we allocate another $b$ budget to it so over all
	we increase the budget by at most $2n \cdot b$. On the other hand, each unit of budget is responsible for two coin tosses (for the $\king$ and its challenger) and so 
	the total number of coin tosses is at most $4n \cdot b$ implying the claim as $b = O(\frac{\ln{(1/\delta)}}{\Delta^2})$. 
\end{proof}

\subsection*{Proof of \Cref{lem:main-pick}}

\begin{lemma*}
	The probability that the most biased coin \coinstar does \emph{not} defeat the $\king$  is at most $(\delta/2)$. 
\end{lemma*}
\begin{proof}
Let $\king$ be any coin other than the most biased coin and suppose the next arriving coin is the most biased one (denoted by $\coinstar$). We can write the probability that $\coinstar$ defeats $\king$ based on the different level $\ell$ of challenges done between the two as follows: 
\begin{align*}
	\Pr\paren{\textnormal{$\coinstar$ loses to $\king$}} &\leq \sum_{\ell=1}^{\infty} \Pr\paren{\textnormal{$\coinstar$ loses to $\king$ at level $\ell \mid \coin$ has not lost until level $\ell-1$}} \\
	&\leq \sum_{\ell=1}^{\infty} 2 \cdot \exp\paren{-\ln{(1/\delta) \cdot r_{\ell}}} \tag{by \Cref{lem:coin-comp} and $s_{\ell}$ number of samples done in level $\ell$} \\
	&< 2\delta \cdot \sum_{\ell=1}^{\infty} \exp\paren{-3^{\ell}} \tag{by definition of $r_\ell = 3^{\ell}$ and since $\ln{(1/\delta)} \cdot r_{\ell} \geq \ln{(1/\delta)} + r_\ell$}\\
	&< (\delta/2) \tag{as this series converges to $<1/10$}
\end{align*}
Since the budget  is finite, $\king$ will  lose to $\coinstar$ in finite time with probability $1-(\delta/2)$. 
\end{proof}

==> related.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex


\section{Related Work}
